Ensemble Spectral Prediction (ESP) Model for Metabolite Annotation

A key challenge in metabolomics is annotating measured spectra from a biological sample with chemical identities. Currently, only a small fraction of measurements can be assigned identities. Two complementary computational approaches have emerged to address the annotation problem: mapping candidate molecules to spectra, and mapping query spectra to molecular candidates. In essence, the candidate molecule with the spectrum that best explains the query spectrum is recommended as the target molecule. Despite candidate ranking being fundamental in both approaches, no prior works utilized rank learning tasks in determining the target molecule. We propose a novel machine learning model, Ensemble Spectral Prediction (ESP), for metabolite annotation. ESP takes advantage of prior neural network-based annotation models that utilize multilayer perceptron (MLP) networks and Graph Neural Networks (GNNs). Based on the ranking results of the MLP and GNN-based models, ESP learns a weighting for the outputs of MLP and GNN spectral predictors to generate a spectral prediction for a query molecule. Importantly, training data is stratified by molecular formula to provide candidate sets during model training. Further, baseline MLP and GNN models are enhanced by considering peak dependencies through multi-head attention mechanism and multi-tasking on spectral topic distributions. ESP improves average rank by 41% and 30% over the MLP and GNN baselines, respectively, demonstrating remarkable performance gain over state-of-the-art neural network approaches. We show that annotation performance, for ESP and other models, is a strong function of the number of molecules in the candidate set and their similarity to the target molecule.

==> fig_rankdiff.tex <==
\begin{figure}%[tbhp]
\centering
\includegraphics[width=.8\linewidth]{figures&tables/rankdiff.png}
\caption{Rank difference among ensemble, MLP and GNN models}
\label{fig:rankdiff}
\end{figure}


==> table2.tex <==
\begin{table*}

\caption{Metabolite annotation evaluation \label{Tab:01}} {
\begin{tabular} {cccccc}
\toprule 
&    Average rank    &    Rank@1    &    Rank@3    &    Rank@5    &    Rank@10 \\

\cmidrule(lr){2-2} \cmidrule(lr){3-6} 

& \multicolumn{1}{c}{\textcolor{blue}{The lower the better}} & \multicolumn{4}{c}{\textcolor{blue}{The higher the better}}\\

\midrule & \multicolumn{5}{c}{A. Predicting MS using fingerprints or molecular graphs}\\ \cmidrule(lr){2-6}
MLP(ECFP) 	                &	14.993	&	0.375	&	0.577	&	0.661	&	0.760\\
GNN	                        &	11.491	&	0.463	&	0.641	&	0.717	&	0.801\\
MLP(ECFP) + Bidirectional	&	9.567	&	0.505	&	0.692	&	0.765	&	0.840\\
GNN + Bidirectional	        &	8.550	&	0.531	&	0.719	&	0.785	&	0.856\\

\cmidrule(lr){1-6} & \multicolumn{5}{c}{B. Predicting LDA topic modeling using MTL}\\ \cmidrule(lr){2-6}

Best MLP + LDA	            &	8.836	&	0.516	&	0.714	&	0.783	&	0.854\\
Best GNN + LDA	            &	8.280	&	0.535	&	0.721	&	0.789	&	0.864\\

\cmidrule(lr){1-6} & \multicolumn{5}{c}{C. Multi-head attention on spectra prediction on top of LDA model}\\ \cmidrule(lr){2-6}

Best MLP + LDA + Attention	    &	8.231	&	0.520	&	0.723	&	0.787	&	0.863\\
Best GNN + LDA + Attention	    &	7.683	&	0.538	&	0.726	&	0.795	&	0.866\\

\cmidrule(lr){1-6} & \multicolumn{5}{c}{D. Ensemble MLP and GNN model with LDA and attention}\\ \cmidrule(lr){2-6}

Ensemble (Best MLP + LDA + Attention, Best GNN + LDA + Attention)	
                            &	6.688	&	0.558	&	0.757	&	0.818	&	0.881\\
                            
\cmidrule(lr){1-6} & \multicolumn{5}{c}{E. Ensemble MLP and GNN model with LDA and attention (using target molecule loss generated label)}\\ \cmidrule(lr){2-6}

Ensemble (using target molecule loss generated label)	
                            &	8.221	&	0.553	&	0.726	&	0.787	&	0.854\\
\bottomrule
\end{tabular}}{}\
\end{table*}



% \begin{table}%[tbhp]
% \centering
% \caption{Comparison of the fitted potential energy surfaces and ab initio benchmark electronic energy calculations}
% \begin{tabular}{lrrr}
% Species & CBS & CV & G3 \\
% \midrule
% 1. Acetaldehyde & 0.0 & 0.0 & 0.0 \\
% 2. Vinyl alcohol & 9.1 & 9.6 & 13.5 \\
% 3. Hydroxyethylidene & 50.8 & 51.2 & 54.0\\
% \bottomrule
% \end{tabular}

% \addtabletext{nomenclature for the TSs refers to the numbered species in the table.}
% \end{table}
